A Machine Learning Approach to Measuring Climate Adaptation

I measure adaptation to climate change by comparing elasticities from short-run and long-run changes in damaging weather. I propose a debiased machine learning approach to flexibly measure these elasticities in panel settings. In a simulation exercise, I show that debiased machine learning has considerable benefits relative to standard machine learning or ordinary least squares, particularly in high-dimensional settings. I then measure adaptation to damaging heat exposure in United States corn and soy production. Using rich sets of temperature and precipitation variation, I find evidence that short-run impacts from damaging heat are significantly offset in the long run. I show that this is because the impacts of long-run changes in heat exposure do not follow the same functional form as short-run shocks to heat exposure.

==> outputs/ag_results/ag_results_table_corn_full_weighted.tex <==
\begin{tabular}{lllcccccc}
\toprule
          &                  & method &        OLS Linear &          OLS Poly &             Lasso &         Lasso DML &              NNet &          NNet DML \\
Variation & Weather & {} &                   &                   &                   &                   &                   &                   \\
\midrule
\multirow{12}{*}{Long-Run} & \multirow{4}{*}{Yearly Linear} & $\theta$ &   -0.0048$^{***}$ &    -0.00109$^{*}$ &  -0.00414$^{***}$ &  -0.00428$^{***}$ &  -0.00357$^{***}$ &  -0.00369$^{***}$ \\
          &                  & \  &        (0.000251) &        (0.000474) &        (0.000404) &        (0.000396) &        (0.000806) &        (0.000811) \\
          &                  & MSE &           0.00239 &           0.00174 &           0.00662 &           0.00662 &           0.00681 &           0.00681 \\
          &                  & N &              2852 &              2852 &              2852 &              2852 &              2852 &              2852 \\
\cline{2-9}
          & \multirow{4}{*}{Yearly Flexible} & $\theta$ &    0.0425$^{***}$ &           0.00779 &         -9.88e-05 &    0.0199$^{***}$ &    0.0168$^{***}$ &    0.0226$^{***}$ \\
          &                  & \  &         (0.00641) &          (0.0141) &         (0.00152) &         (0.00273) &         (0.00361) &         (0.00306) \\
          &                  & MSE &           0.00165 &          0.000471 &           0.00561 &           0.00561 &            0.0063 &            0.0063 \\
          &                  & N &              2852 &              2852 &              2852 &              2852 &              2852 &              2852 \\
\cline{2-9}
          & \multirow{4}{*}{Monthly Flexible} & $\theta$ &      0.0154$^{*}$ &         -1.24e+04 &  -0.00168$^{***}$ &          -0.00349 &          0.000632 &          0.000126 \\
          &                  & \  &         (0.00698) &         (2.7e+05) &        (0.000453) &         (0.00268) &        (0.000946) &         (0.00256) \\
          &                  & MSE &          0.000698 &          1.09e-06 &           0.00547 &           0.00547 &           0.00534 &           0.00534 \\
          &                  & N &              2852 &              2852 &              2852 &              2852 &              2852 &              2852 \\
\cline{1-9}
\cline{2-9}
\multirow{12}{*}{Short-Run} & \multirow{4}{*}{Yearly Linear} & $\theta$ &  -0.00622$^{***}$ &  -0.00548$^{***}$ &  -0.00548$^{***}$ &  -0.00549$^{***}$ &  -0.00603$^{***}$ &  -0.00606$^{***}$ \\
          &                  & \  &        (9.89e-05) &        (0.000111) &        (0.000112) &        (0.000112) &        (0.000555) &        (0.000374) \\
          &                  & MSE &            0.0195 &            0.0178 &            0.0381 &            0.0381 &             0.038 &             0.038 \\
          &                  & N &             38637 &             38637 &             38637 &             38637 &             38637 &             38637 \\
\cline{2-9}
          & \multirow{4}{*}{Yearly Flexible} & $\theta$ &  -0.00698$^{***}$ &   -0.00343$^{**}$ &   -0.0048$^{***}$ &  -0.00425$^{***}$ &  -0.00467$^{***}$ &   -0.0046$^{***}$ \\
          &                  & \  &         (0.00116) &         (0.00109) &         (0.00131) &        (0.000914) &        (0.000591) &        (0.000713) \\
          &                  & MSE &             0.019 &            0.0149 &            0.0373 &            0.0373 &            0.0376 &            0.0376 \\
          &                  & N &             38637 &             38637 &             38637 &             38637 &             38637 &             38637 \\
\cline{2-9}
          & \multirow{4}{*}{Monthly Flexible} & $\theta$ &  -0.00762$^{***}$ &              5.52 &  -0.00217$^{***}$ &  -0.00222$^{***}$ &  -0.00454$^{***}$ &  -0.00479$^{***}$ \\
          &                  & \  &         (0.00105) &             (128) &        (0.000199) &        (0.000361) &        (0.000669) &        (0.000746) \\
          &                  & MSE &            0.0162 &             0.011 &            0.0338 &            0.0338 &            0.0332 &            0.0332 \\
          &                  & N &             38637 &             38637 &             38637 &             38637 &             38637 &             38637 \\
\bottomrule
\end{tabular}


==> outputs/ag_results/ag_results_table_soy_full_weighted.tex <==
\begin{tabular}{lllcccccc}
\toprule
          &                  & method &        OLS Linear &          OLS Poly &             Lasso &         Lasso DML &              NNet &          NNet DML \\
Variation & Weather & {} &                   &                   &                   &                   &                   &                   \\
\midrule
\multirow{12}{*}{Long-Run} & \multirow{4}{*}{Yearly Linear} & $\theta$ &  -0.00325$^{***}$ &   -0.0029$^{***}$ &   -0.0054$^{***}$ &  -0.00553$^{***}$ &  -0.00333$^{***}$ &  -0.00365$^{***}$ \\
          &                  & \  &        (0.000265) &        (0.000502) &        (0.000312) &         (0.00031) &        (0.000598) &        (0.000551) \\
          &                  & MSE &           0.00353 &           0.00226 &           0.00555 &           0.00555 &             0.006 &             0.006 \\
          &                  & N &              2423 &              2423 &              2423 &              2423 &              2423 &              2423 \\
\cline{2-9}
          & \multirow{4}{*}{Yearly Flexible} & $\theta$ &           0.00216 &           -0.0135 &  -0.00164$^{***}$ &   0.00815$^{***}$ &      0.014$^{**}$ &    0.00912$^{**}$ \\
          &                  & \  &         (0.00714) &           (0.027) &         (0.00025) &          (0.0019) &           (0.005) &         (0.00289) \\
          &                  & MSE &           0.00188 &          0.000428 &           0.00514 &           0.00514 &           0.00633 &           0.00633 \\
          &                  & N &              2423 &              2423 &              2423 &              2423 &              2423 &              2423 \\
\cline{2-9}
          & \multirow{4}{*}{Monthly Flexible} & $\theta$ &           0.00538 &           0.00611 &  -0.00208$^{***}$ &           0.00331 &    0.00426$^{**}$ &            0.0033 \\
          &                  & \  &         (0.00795) &          (0.0592) &        (0.000281) &         (0.00314) &         (0.00148) &         (0.00348) \\
          &                  & MSE &           0.00078 &          2.85e-11 &           0.00438 &           0.00438 &           0.00468 &           0.00468 \\
          &                  & N &              2423 &              2423 &              2423 &              2423 &              2423 &              2423 \\
\cline{1-9}
\cline{2-9}
\multirow{12}{*}{Short-Run} & \multirow{4}{*}{Yearly Linear} & $\theta$ &  -0.00555$^{***}$ &  -0.00429$^{***}$ &  -0.00432$^{***}$ &  -0.00432$^{***}$ &  -0.00526$^{***}$ &  -0.00539$^{***}$ \\
          &                  & \  &        (6.35e-05) &        (8.21e-05) &         (0.00026) &        (0.000265) &        (0.000407) &        (0.000293) \\
          &                  & MSE &            0.0187 &            0.0168 &            0.0305 &            0.0305 &            0.0302 &            0.0302 \\
          &                  & N &             33812 &             33812 &             33812 &             33812 &             33812 &             33812 \\
\cline{2-9}
          & \multirow{4}{*}{Yearly Flexible} & $\theta$ &  -0.00744$^{***}$ &  -0.00631$^{***}$ &  -0.00461$^{***}$ &  -0.00564$^{***}$ &  -0.00596$^{***}$ &  -0.00637$^{***}$ \\
          &                  & \  &        (0.000978) &         (0.00117) &         (0.00134) &        (0.000746) &         (0.00063) &        (0.000688) \\
          &                  & MSE &            0.0181 &            0.0142 &            0.0296 &            0.0296 &            0.0296 &            0.0296 \\
          &                  & N &             33812 &             33812 &             33812 &             33812 &             33812 &             33812 \\
\cline{2-9}
          & \multirow{4}{*}{Monthly Flexible} & $\theta$ &  -0.00737$^{***}$ &         -8.53e+04 &  -0.00413$^{***}$ &  -0.00372$^{***}$ &  -0.00543$^{***}$ &  -0.00506$^{***}$ \\
          &                  & \  &         (0.00096) &        (9.56e+05) &        (0.000182) &        (0.000354) &         (0.00051) &         (0.00063) \\
          &                  & MSE &            0.0146 &           0.00974 &            0.0257 &            0.0257 &            0.0252 &            0.0252 \\
          &                  & N &             33812 &             33812 &             33812 &             33812 &             33812 &             33812 \\
\bottomrule
\end{tabular}


==> outputs/ag_results/ag_results_table_weighted.tex <==
\begin{tabular}{lllccc|ccc}
\toprule
    &                  & {} & \multicolumn{3}{c}{Long-Run} & \multicolumn{3}{c}{Short-Run} \\
    &                  & method &        OLS Linear &         Lasso DML &          NNet DML &        OLS Linear &         Lasso DML &          NNet DML \\
Crop & Weather & {} &                   &                   &                   &                   &                   &                   \\
\midrule
\multirow{12}{*}{Corn} & \multirow{4}{*}{Yearly Linear} & $\theta$ &   -0.0048$^{***}$ &  -0.00428$^{***}$ &  -0.00369$^{***}$ &  -0.00622$^{***}$ &  -0.00549$^{***}$ &  -0.00606$^{***}$ \\
    &                  & \  &        (0.000251) &        (0.000396) &        (0.000811) &        (9.89e-05) &        (0.000112) &        (0.000374) \\
    &                  & MSE &           0.00239 &           0.00662 &           0.00681 &            0.0195 &            0.0381 &             0.038 \\
    &                  & N &              2852 &              2852 &              2852 &             38637 &             38637 &             38637 \\
\cline{2-9}
    & \multirow{4}{*}{Yearly Flexible} & $\theta$ &    0.0425$^{***}$ &    0.0199$^{***}$ &    0.0226$^{***}$ &  -0.00698$^{***}$ &  -0.00425$^{***}$ &   -0.0046$^{***}$ \\
    &                  & \  &         (0.00641) &         (0.00273) &         (0.00306) &         (0.00116) &        (0.000914) &        (0.000713) \\
    &                  & MSE &           0.00165 &           0.00561 &            0.0063 &             0.019 &            0.0373 &            0.0376 \\
    &                  & N &              2852 &              2852 &              2852 &             38637 &             38637 &             38637 \\
\cline{2-9}
    & \multirow{4}{*}{Monthly Flexible} & $\theta$ &      0.0154$^{*}$ &          -0.00349 &          0.000126 &  -0.00762$^{***}$ &  -0.00222$^{***}$ &  -0.00479$^{***}$ \\
    &                  & \  &         (0.00698) &         (0.00268) &         (0.00256) &         (0.00105) &        (0.000361) &        (0.000746) \\
    &                  & MSE &          0.000698 &           0.00547 &           0.00534 &            0.0162 &            0.0338 &            0.0332 \\
    &                  & N &              2852 &              2852 &              2852 &             38637 &             38637 &             38637 \\
\cline{1-9}
\cline{2-9}
\multirow{12}{*}{Soy} & \multirow{4}{*}{Yearly Linear} & $\theta$ &  -0.00325$^{***}$ &  -0.00553$^{***}$ &  -0.00365$^{***}$ &  -0.00555$^{***}$ &  -0.00432$^{***}$ &  -0.00539$^{***}$ \\
    &                  & \  &        (0.000265) &         (0.00031) &        (0.000551) &        (6.35e-05) &        (0.000265) &        (0.000293) \\
    &                  & MSE &           0.00353 &           0.00555 &             0.006 &            0.0187 &            0.0305 &            0.0302 \\
    &                  & N &              2423 &              2423 &              2423 &             33812 &             33812 &             33812 \\
\cline{2-9}
    & \multirow{4}{*}{Yearly Flexible} & $\theta$ &           0.00216 &   0.00815$^{***}$ &    0.00912$^{**}$ &  -0.00744$^{***}$ &  -0.00564$^{***}$ &  -0.00637$^{***}$ \\
    &                  & \  &         (0.00714) &          (0.0019) &         (0.00289) &        (0.000978) &        (0.000746) &        (0.000688) \\
    &                  & MSE &           0.00188 &           0.00514 &           0.00633 &            0.0181 &            0.0296 &            0.0296 \\
    &                  & N &              2423 &              2423 &              2423 &             33812 &             33812 &             33812 \\
\cline{2-9}
    & \multirow{4}{*}{Monthly Flexible} & $\theta$ &           0.00538 &           0.00331 &            0.0033 &  -0.00737$^{***}$ &  -0.00372$^{***}$ &  -0.00506$^{***}$ \\
    &                  & \  &         (0.00795) &         (0.00314) &         (0.00348) &         (0.00096) &        (0.000354) &         (0.00063) \\
    &                  & MSE &           0.00078 &           0.00438 &           0.00468 &            0.0146 &            0.0257 &            0.0252 \\
    &                  & N &              2423 &              2423 &              2423 &             33812 &             33812 &             33812 \\
\bottomrule
\end{tabular}

